Outcome coding choice in randomized trials of programs to reduce violence

Over the last decade, the number of randomized trials of programs to reduce intimate partner violence (IPV) has grown precipitously. However, most trials continue to measure and code violence using standards originally designed for global prevalence surveys. This choice may have consequences in terms of bias, power, and efficiency of trial estimates and may limit what we can learn about how programs are working. In this paper, we return to first principles to develop a generative model for violence reduction. We then use this model to better understand trade-offs in outcome coding choices via simulation. We re-analyze results from seven recent trials in Southern and Eastern Africa to highlight some of our findings. We conclude with a discussion of key take-aways for trialists.

==> IPV Measurement-2/setup.tex <==
\usepackage{amssymb,amsmath,amsfonts,eurosym,geometry,ulem,graphicx,caption,color,setspace,sectsty,comment,footmisc,caption,pdflscape,subcaption,array,hyperref,booktabs, threeparttable}

\usepackage[affil-it]{authblk}
\usepackage[
backend=biber,
style=nature,
sorting=none,
doi=false,
isbn=false,
url=false,
eprint=false,
date=year
]{biblatex}

\normalem

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut

\onehalfspacing
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}{Proposition}
\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

\newtheorem{hyp}{Hypothesis}
\newtheorem{subhyp}{Hypothesis}[hyp]
\renewcommand{\thesubhyp}{\thehyp\alph{subhyp}}

\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\arraybackslash\hspace{0pt}}m{#1}}

\geometry{left=1.0in,right=1.0in,top=1.0in,bottom=1.0in}

==> IPV Measurement-2/tables/table1.tex <==
\begin{table}

\caption{Simulation results based on Becoming One study in Uganda.\label{tab:b1_sims}}
\centering
\fontsize{7}{9}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lcccccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{All acts} & \multicolumn{4}{c}{Physical only} & \multicolumn{4}{c}{Sexual only} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9} \cmidrule(l{3pt}r{3pt}){10-13}
 & Bias & RMSE & Power & Coverage & Bias & RMSE & Power & Coverage & Bias & RMSE & Power & Coverage\\
\midrule
\addlinespace[0.3em]
\multicolumn{13}{l}{\textbf{Cessation only}}\\
\hspace{1em}$Y_{binary}$ & 0 & 0.020 & 1.000 & 0.957 & 0 & 0.022 & 0.289 & 0.946 & 0 & 0.021 & 0.682 & 0.956\\
\hspace{1em}$Y_{sum}$ & 0 & 0.006 & 0.972 & 0.964 & 0 & 0.006 & 0.511 & 0.957 & 0 & 0.006 & 0.375 & 0.959\\
\addlinespace[0.3em]
\multicolumn{13}{l}{\textbf{Cessation + reduction}}\\
\hspace{1em}$Y_{binary}$ & 0 & 0.021 & 0.488 & 0.949 & 0 & 0.022 & 0.071 & 0.953 & 0 & 0.022 & 0.125 & 0.953\\
\hspace{1em}$Y_{sum}$ & 0 & 0.006 & 0.551 & 0.961 & 0 & 0.006 & 0.194 & 0.960 & 0 & 0.006 & 0.152 & 0.955\\
\addlinespace[0.3em]
\multicolumn{13}{l}{\textbf{Reduction only}}\\
\hspace{1em}$Y_{binary}$ & 0 & 0.022 & 0.048 & 0.952 & 0 & 0.022 & 0.048 & 0.952 & 0 & 0.022 & 0.048 & 0.952\\
\hspace{1em}$Y_{sum}$ & 0 & 0.006 & 0.255 & 0.957 & 0 & 0.006 & 0.103 & 0.954 & 0 & 0.006 & 0.096 & 0.957\\
\addlinespace[0.3em]
\multicolumn{13}{l}{\textbf{Cessation + reduction + increase}}\\
\hspace{1em}$Y_{binary}$ & 0 & 0.021 & 0.481 & 0.953 & 0 & 0.022 & 0.072 & 0.949 & 0 & 0.022 & 0.127 & 0.955\\
\hspace{1em}$Y_{sum}$ & 0 & 0.006 & 0.350 & 0.957 & 0 & 0.006 & 0.136 & 0.956 & 0 & 0.006 & 0.113 & 0.953\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \textit{Notes:} 
\item Monte carlo performance estimates based on 1,000 simulated assignments and 100 bootstrap samples. 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> IPV Measurement-2/tables/tablea1.tex <==
\begin{table}[b]

\caption{Full results for monte carlo simulation of power using DHS data.\label{tab:dhs_sims_power}}
\centering
\fontsize{7}{9}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lp{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{b{1.4cm}}{\centering Ukraine (2007)} & \multicolumn{2}{b{1.4cm}}{\centering Nepal (2016)} & \multicolumn{2}{b{1.4cm}}{\centering Philippines (2017)} & \multicolumn{2}{b{1.4cm}}{\centering Peru (2012)} & \multicolumn{2}{b{1.4cm}}{\centering Dominican Republic (2013)} & \multicolumn{2}{b{1.4cm}}{\centering Tajikistan (2017)} & \multicolumn{2}{b{1.4cm}}{\centering Uganda (2016)} & \multicolumn{2}{b{1.4cm}}{\centering Nigeria (2013)} & \multicolumn{2}{b{1.4cm}}{\centering Papua New Guinea (2016)} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13} \cmidrule(l{3pt}r{3pt}){14-15} \cmidrule(l{3pt}r{3pt}){16-17} \cmidrule(l{3pt}r{3pt}){18-19}
 & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$ & $Y_{binary}$ & $Y_{sum}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{All acts}}\\
\hspace{1em}cessation only & 0.971 & 0.807 & 0.981 & 0.781 & 0.886 & 0.647 & 1.000 & 1.000 & 1.000 & 0.985 & 0.793 & 0.469 & 0.976 & 0.862 & 1.000 & 0.992 & 0.725 & 0.535\\
\hspace{1em}cessation + reduction & 0.258 & 0.415 & 0.250 & 0.294 & 0.168 & 0.267 & 0.703 & 0.888 & 0.437 & 0.482 & 0.137 & 0.159 & 0.246 & 0.419 & 0.562 & 0.671 & 0.138 & 0.257\\
\hspace{1em}reduction only & 0.050 & 0.190 & 0.045 & 0.125 & 0.060 & 0.130 & 0.040 & 0.569 & 0.056 & 0.155 & 0.047 & 0.081 & 0.064 & 0.206 & 0.056 & 0.335 & 0.053 & 0.121\\
\hspace{1em}cessation + reduction + increase & 0.232 & 0.240 & 0.255 & 0.162 & 0.177 & 0.170 & 0.660 & 0.636 & 0.430 & 0.248 & 0.148 & 0.113 & 0.253 & 0.251 & 0.569 & 0.415 & 0.156 & 0.156\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{Physical only}}\\
\hspace{1em}cessation only & 0.903 & 0.705 & 0.740 & 0.573 & 0.577 & 0.456 & 0.972 & 0.984 & 0.988 & 0.937 & 0.426 & 0.310 & 0.955 & 0.801 & 0.922 & 0.917 & 0.596 & 0.489\\
\hspace{1em}cessation + reduction & 0.182 & 0.321 & 0.138 & 0.191 & 0.102 & 0.163 & 0.232 & 0.720 & 0.306 & 0.398 & 0.090 & 0.129 & 0.212 & 0.360 & 0.204 & 0.434 & 0.102 & 0.204\\
\hspace{1em}reduction only & 0.044 & 0.161 & 0.042 & 0.089 & 0.050 & 0.098 & 0.060 & 0.380 & 0.065 & 0.126 & 0.060 & 0.079 & 0.061 & 0.209 & 0.040 & 0.162 & 0.040 & 0.124\\
\hspace{1em}cessation + reduction + increase & 0.186 & 0.213 & 0.121 & 0.115 & 0.117 & 0.121 & 0.253 & 0.436 & 0.290 & 0.211 & 0.077 & 0.088 & 0.208 & 0.231 & 0.203 & 0.233 & 0.090 & 0.126\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{Sexual only}}\\
\hspace{1em}cessation only & 0.041 & 0.058 & 0.050 & 0.080 & 0.069 & 0.066 & 0.065 & 0.191 & 0.047 & 0.070 & 0.049 & 0.062 & 0.046 & 0.060 & 0.124 & 0.198 & 0.045 & 0.050\\
\hspace{1em}cessation + reduction & 0.046 & 0.043 & 0.056 & 0.063 & 0.049 & 0.071 & 0.058 & 0.099 & 0.052 & 0.057 & 0.054 & 0.058 & 0.053 & 0.046 & 0.067 & 0.109 & 0.048 & 0.053\\
\hspace{1em}reduction only & 0.045 & 0.044 & 0.055 & 0.052 & 0.052 & 0.050 & 0.060 & 0.075 & 0.058 & 0.059 & 0.049 & 0.045 & 0.071 & 0.052 & 0.062 & 0.083 & 0.052 & 0.053\\
\hspace{1em}cessation + reduction + increase & 0.040 & 0.057 & 0.050 & 0.051 & 0.046 & 0.052 & 0.043 & 0.081 & 0.052 & 0.045 & 0.059 & 0.057 & 0.045 & 0.055 & 0.064 & 0.084 & 0.056 & 0.051\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{Moderate only}}\\
\hspace{1em}cessation only & 0.227 & 0.210 & 0.230 & 0.175 & 0.176 & 0.167 & 0.203 & 0.383 & 0.376 & 0.482 & 0.143 & 0.117 & 0.535 & 0.433 & 0.256 & 0.346 & 0.195 & 0.204\\
\hspace{1em}cessation + reduction & 0.055 & 0.104 & 0.072 & 0.071 & 0.071 & 0.099 & 0.056 & 0.189 & 0.063 & 0.140 & 0.065 & 0.068 & 0.088 & 0.171 & 0.066 & 0.128 & 0.078 & 0.104\\
\hspace{1em}reduction only & 0.060 & 0.091 & 0.048 & 0.054 & 0.054 & 0.069 & 0.052 & 0.089 & 0.053 & 0.071 & 0.063 & 0.051 & 0.058 & 0.126 & 0.053 & 0.069 & 0.054 & 0.073\\
\hspace{1em}cessation + reduction + increase & 0.076 & 0.095 & 0.060 & 0.066 & 0.063 & 0.073 & 0.072 & 0.111 & 0.078 & 0.093 & 0.048 & 0.055 & 0.106 & 0.135 & 0.063 & 0.102 & 0.058 & 0.082\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \textit{Notes:} 
\item Monte carlo performance estimates based on 1,000 simulated assignments and 100 bootstrap samples. 
\end{tablenotes}
\end{threeparttable}
\end{table}

